Chart2SVG: Editable SVG Generation from Raster Chart Images

We present Chart2SVG, a multimodal large language model that converts static raster charts into structurally organized, semantically enriched SVGs that support programmatic editing. By incorporating chart-specific semantic tokens into a vision-language model, Chart2SVG captures both geometric primitives and their functional roles. To support robust structural recovery, we introduce Beagle+, a dataset of 33K canonicalized and structurally distilled chart samples. Our approach combines specialized training objectives with a rendering-aware post-training phase, producing SVGs that are both visually accurate and structurally consistent. To facilitate higher-level manipulations, we construct a Chart Structure Graph (CSG) that exposes visual dependencies, enabling tasks such as interactive exploration, chart repurposing, and layout reuse. Experiments show that Chart2SVG substantially outperforms baselines in reconstruction fidelity and downstream editing utility, advancing the development of intelligent and interactive visualization tools.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023
modified by Matt Brehmer, Feburary 2024
modified by Tobias Isenberg, December 2025

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
figs/           - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g., R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/0_abstract_refine.tex <==
Charts are indispensable for conveying complex data insights, yet adapting existing visualizations to evolving requirements remains a significant bottleneck in the data visualization lifecycle. While static raster charts are ubiquitous in reports and publications, editing them—ranging from local data updates to global style optimizations—typically requires manual reconstruction or error-prone pixel-level manipulation. In this paper, we propose a novel framework for automated, high-fidelity chart editing by bridging the gap between visual perception and structural manipulation in the SVG representation space. Our approach first employs a Vision-Language Model (VLM), Qwen3-VL, to reconstruct SVG charts from raster inputs. To ensure geometric precision and code validity, we introduce an SVG normalization pipeline and optimize the model using rendering-aware Group Relative Policy Optimization (GRPO), which incorporates execution-based visual feedback. To enable controllable editing, we lift the reconstructed primitives into a structured semantic representation, organizing chart components (e.g., axes, legends, data marks) into a chart dependency graph. This graph preserves essential hierarchical and cross-component constraints, allowing a Large Language Model (LLM) to interpret natural language intent and execute coordinated edit plans. Quantitative and qualitative evaluations demonstrate that our framework significantly improves reconstruction fidelity and provides a robust, intuitive mechanism for both local adjustments and complex global chart transformations.




==> sections/1_intro.tex <==
\section{Introduction}

% ================================================
% \textbf{Paragraph 1: Background and Motivation}

% A long-standing pain point in the visualization community:
% Charts are often shared only as raster images. While this makes them easy to view and distribute, it makes them difficult to edit and reuse (restyle, resize, or update with new data).
% ================================================


Charts serve as a crucial medium for information communication, playing an indispensable role in conveying complex data insights across diverse fields such as scientific research, business analytics, and journalism. Unlike raw data tables, charts leverage visual encodings to transform abstract numbers into intuitive patterns, enabling users to rapidly perceive trends, clusters, and anomalies. As the volume and complexity of data grow, the ubiquity of charts continues to rise, making them a fundamental carrier of knowledge in the information age. However, data visualization is rarely a static, one-time process; it is inherently iterative. While charts are heavily consumed as static raster images in scientific papers and reports, adapting them to new contexts—such as updating data, restyling for accessibility, or adapting layouts—remains a severe bottleneck.

Despite the maturity of chart authoring tools, the necessity for chart editing—modifying existing visualizations—remains a persistent and critical challenge in real-world scenarios. Unlike chart creation, chart editing focuses on refining an existing artifact to better suit evolving requirements contexts. These modifications can range from local adjustments, such as correcting a mislabeled axis or updating a specific data point, to global optimizations, such as altering the color theme for accessibility or switching the chart type to improve clarity. This iterative process is fundamental to the lifecycle of data visualization, ensuring that charts remain accurate and effective as contexts change.~\cite{jung2017chartsense,kim2020answering}

To achieve chart editing, traditional methods typically involve a two-step workflow: users must first utilize professional graphic design tools (e.g., Adobe Illustrator, Inkscape) to reconstruct or extract the SVG code that contains the chart’s structural information, and then perform targeted modifications on the SVG to satisfy new requirements~\cite{2017-vega-lite}. However, this approach imposes significant barriers; it demands that users possess specialized knowledge of vector editing tools and a deep understanding of SVG syntax. Consequently, the process is often tedious, inefficient, and prone to manual errors, especially for users without a design background. With the advent of Multimodal Large Language Models (MLLMs), some approaches attempt to bypass this complexity by inputting prompts to directly modify chart images at the pixel level. Nevertheless, charts are inherently information-dense images characterized by complex structures and strict logic. Direct pixel-level modification struggles to preserve the fine-grained structural details of charts, often resulting in low precision. Furthermore, this approach frequently suffers from text distortion, geometric deformation, and “data hallucinations,” where the modified chart fails to maintain data integrity or loses the scalability inherent to vector graphics. Therefore, to achieve accurate and high-fidelity chart editing, it is essential to operate within the corresponding SVG representation space. 
%Recent progress in vision-language models (VLMs) and large language models (LLMs) suggests that this gap may now be bridgeable. 
%Emerging work has shown that these foundation models can generate SVG from visual or textual inputs~\cite{xing2025empowering,rodriguez2025starvector}, making image-to-SVG recovery~\cite{rodriguez2025rendering} and language-guided editing~\cite{masson2024directgpt} increasingly feasible.

However, realizing automated chart editing within the SVG space faces two formidable challenges. The first challenge lies in the diversity and heterogeneity of charts. Charts vary widely in types (e.g., bar, line, scatter) and visual styles. Crucially, they encapsulate rich structured semantic information—such as the correspondence between data series and visual elements—which goes beyond simple geometric shapes. Existing SVG generation methods~\cite{yang2025omnisvgunifiedscalablevector, wang2026internsvgunifiedsvgtasks, reddy2021im2vec} perform a flattening process on the SVGs, removing a large number of attributes and structural tags, often struggle to capture this depth of information, making it difficult to efficiently recover the corresponding SVG structure from a static chart image. Constructing a universal and standardized process for structure extraction remains a bottleneck. The second challenge pertains to the modification efficacy. Even with the SVG representation obtained, determining how to rapidly locate the target elements and adapt them to specific editing requirements—particularly for complex global optimizations—directly impacts the efficiency and usability of the editing task~\cite{snyder2023divi, masson2024directgpt}.

To address these challenges, this paper proposes a novel framework comprising an SVG generation pre-trained model and an LLM-based SVG-assisted editing mechanism. By bridging the gap between visual perception and structural manipulation, our framework aims to facilitate accurate and efficient chart editing.

%In the first stage, we fine-tune a VLM (instantiated with Qwen3-VL~\cite{bai2025qwen3}) to recover SVGs from raster inputs. Recognizing that charts adhere to strict geometric and stylistic conventions, we introduce an SVG normalization pipeline to canonicalize raw SVGs, reducing unnecessary structural variability and stabilizing training. Beyond standard supervised fine-tuning (SFT), we employ rendering-aware GRPO~\cite{shao2024deepseekmath,rodriguez2025rendering} with a composite reward measuring pixel fidelity, structural integrity, and code validity. This addresses the data logic specificity of charts, ensuring the generated SVGs are not only textually plausible but also executable and visually faithful.
In the first stage, we train a VLM, instantiated with Qwen3-VL~\cite{bai2025qwen3}, to recover SVG charts from raster inputs. To account for the strict geometric and stylistic conventions of charts, we introduce an SVG normalization pipeline that canonicalizes raw SVGs by removing structural artifacts and standardizing geometry, coordinate systems, and styling, thereby reducing unnecessary variability and improving training stability. 
We then perform supervised fine-tuning (SFT) on a large-scale normalized chart image--SVG dataset. 
However, since SFT operates purely in token space, it does not directly assess the rendered appearance of generated SVGs and may produce invalid or non-renderable outputs. 
To address this limitation, we further optimize the model with rendering-aware GRPO ~\cite{shao2024deepseekmath,rodriguez2025rendering}, which incorporates execution-based visual feedback. 
The reward combines pixel-level fidelity, structural consistency, and SVG code validity, encouraging outputs that are both visually faithful and executable.


%In the second stage, to manage the hierarchical semantics inherent in charts, we parse the reconstructed SVG into a chart dependency graph. This structure aggregates low-level primitives into semantic components (e.g., axes, legends) based on geometric cues, modeling the coupling relationships between elements. Guided by this graph, an LLM interprets user intent and generates structured edit plans that respect dependency constraints (e.g., synchronizing legend markers with series colors). This approach effectively supports complex global optimizations that require coordinated modifications, bridging the gap between high-level user intent and low-level SVG manipulation.
In the second stage, rather than treating reconstructed SVGs as flat collections of graphical primitives, we lift them into a structured semantic representation to enable reliable and controllable editing. 
Specifically, we first identify the semantic roles of primitives and group them into higher-level chart components (e.g., axes, bar groups, ticks, and legends). 
This decomposition leverages both code-level cues, such as grouping structures and class attributes, and geometric and stylistic regularities, including alignment, repetition, proximity, and visual similarity. 
Based on this semantic organization, we further construct a chart dependency graph, where nodes represent components, primitives, and editable attributes, and edges encode both hierarchical containment and cross-component correspondences (e.g., alignment between data marks and axis ticks) that should be preserved during editing. 
Guided by this structured representation, an LLM interprets user intent and generates structured edit plans subject to these dependency constraints. 
This design supports not only precise local modifications within individual components, but also complex global updates that require coordinated changes across multiple related elements, effectively bridging high-level user intent and low-level SVG manipulation.


%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Charts are a primary medium for communicating quantitative information in scientific papers, news articles, and reports. 
% However, they are frequently shared only as raster images. While rasterization makes charts easy to view and distribute, it also strips away the structure needed for editing and reuse. 
% Once a chart is reduced to pixels, common operations such as restyling elements and adjusting layout become difficult and often require manual recreation from scratch. 
% This disconnect between how charts are consumed and how they can be practically edited remains a long-standing pain point for visualization workflows~\cite{jung2017chartsense,kim2020answering}.

% Visualization authoring often begins with examples. Designers frequently search for existing visualizations, draw inspiration from them, and adapt them to their own data and communication goals~\cite{bako2022understanding}. In practice, however, many charts are only available as raster images. While easy to view and distribute, raster charts discard the structural information needed for editing and reuse, making it difficult to transform an existing chart into the form a user actually wants.

 
% ================================================
% \textbf{Paragraph 2: Limitations of prior work}

% Prior visualization reverse-engineering work [Jeffery Heer] focused on recovering data or specifications from chart images, often through OCR and heuristic-heavy pipelines. Meanwhile, SVG editing systems like [DIVI] and [Mystique] assume SVG is already available.
% Neither fully solves the problem of recovering raster charts into forms that support practical downstream editing and reuse.
% ================================================

% Prior work has addressed parts of this problem in isolation.
% Research on visualization reverse engineering has studied how to recover data tables and visual encodings from chart images, often through OCR, detection models, and heuristic analysis pipelines~\cite{poco2017reverse,savva2011revision}. 
% These methods are valuable for chart interpretation, but they typically target analytical recovery rather than editable vector graphics reconstruction. 
% Conversely, SVG-based chart interaction systems~\cite{snyder2023divi,chen2023mystique} assume that a structured vector graphic is already available.
% As a result, existing approaches leave a critical gap: 
% neither fully solves the problem of recovering raster charts into forms that support practical downstream editing and reuse.


% ================================================
% \textbf{Paragraph 3: Opportunities and Challenges}

% Recent advances in VLMs and LLMs make image-to-SVG recovery [LLM4SVG, StarVector, LayerSVG] and language-guided editing [DirectGPT] increasingly feasible.

% However, raw SVG remains ill-suited for both learning and interaction:
% (1) SVGs found in the wild often contain heterogeneous structure, redundant elements, and tool-specific artifacts that complicate model training.
% (2) Reconstructed SVGs are too low-level for practical chart editing because they expose graphical primitives rather than semantic units such as bar groups, axis ticks, legends, and gridlines, which users typically target. This mismatch makes direct LLM-based editing less reliable, since the model must first infer chart structure in order to identify the right elements and propagate edits consistently.
% ================================================

% Recent progress in vision-language models (VLMs) and large language models (LLMs) suggests that this gap may now be bridgeable. 
% Emerging work has shown that these foundation models can generate SVG from visual or textual inputs~\cite{xing2025empowering,rodriguez2025starvector}, making image-to-SVG recovery~\cite{rodriguez2025rendering} and language-guided editing~\cite{masson2024directgpt} increasingly feasible.
% However, directly applying these advances to charts remains challenging. 
% On the reconstruction side, raw SVG collected from the web is highly heterogeneous, often containing nested transforms, redundant elements, and tool-specific artifacts that complicate model learning and reduce reconstruction fidelity. 
% Version 1
% Second, even when reconstruction succeeds, the resulting SVG is typically represented as low-level graphical primitives rather than semantic chart components and their relationships. 
% However, practical chart editing depends on both: users edit bars, ticks, legends, and gridlines as meaningful units, and many edits require coordinated updates across these components to preserve global consistency.
% Without an explicit modeling of semantic hierarchy and cross-component dependencies, direct LLM-based editing on raw primitives is unreliable and often produces incoherent modifications.
% Version 2
% On the editing side, raw SVG remains too low-level to serve as a practical editing interface since it mainly exposes graphical primitives.
% Users, however, typically express edits over higher-level chart components, and many operations must be propagated consistently across semantically related elements such as data marks, axis ticks, and legend entries.
% Therefore, editable chart recovery requires not only visual reconstruction, but also sufficient semantic structure to support consistent editing.


% ================================================
% \textbf{Paragraph 4: System overview}

% We address this gap with a system that reconstructs raster charts into SVG, infers chart semantics, and enables direct chart-level editing.
% Stage 1: reconstructs chart SVG from the input image by training a VLM (raw SVG normalization, SFT, rendering-aware GRPO).

% Rather than treating chart reconstruction as an end in itself, our goal is to support downstream applications such as component-level restyling, layout adjustment, and chart reuse with new data.
% To this end,
% Stage 2: lifts the reconstructed SVG into semantic chart components and supports group-wise editing operations through LLM-guided direct manipulation.
% ================================================

% In this paper, we address these challenges with a system that reconstructs raster charts into editable SVG, infers structured chart semantics, and enables language-guided direct chart-level editing. 
% Our system consists of two stages. 
% In the first stage, we train a VLM, instantiated with Qwen3-VL~\cite{bai2025qwen3}, to recover SVG charts from raster inputs.
% A key ingredient is an SVG normalization pipeline that canonicalizes raw chart SVG by removing structural artifacts and standardizing geometry, coordinate systems, and styling conventions, thereby reducing unnecessary variability in the target learning space and improving training stability.
% Following standard foundation-model post-training practice, we perform supervised fine-tuning (SFT) on a large-scale normalized chart image--SVG dataset.
% However, because SFT operates only in token space, it does not directly evaluate the rendered appearance of generated SVG and may still produce invalid or non-renderable code.
% We therefore further optimize the model with rendering-aware GRPO~\cite{shao2024deepseekmath,rodriguez2025rendering}, which closes the loop through execution-based visual feedback.
% Its reward combines both pixel- and structural-level measures of rendered image fidelity together with an SVG code validity term, encouraging outputs that are both visually faithful and executable.

%Rather than treating chart reconstruction as an end, our goal is to make raster charts practically editable under language instructions.
% To this end, the second stage lifts reconstructed SVGs from low-level graphical primitives into a semantic graph of chart components for reliable language-guided editing.
% This decomposition combines code-level cues, such as grouping structure and class names, with geometric regularities including alignment, repetition, and containment to recover components such as bar groups, ticks, and legends.
% It recovers higher-level semantic components by exploiting geometric and stylistic cues such as alignment, repetition, proximity, and visual similarity.
%To this end, the second stage identifies the semantic roles of graphical primitives in the reconstructed SVG and groups them into higher-level chart components by leveraging geometric and stylistic cues such as alignment, repetition, proximity, and visual similarity.
% On top of this semantic structure, it builds a chart dependency graph that captures not only component hierarchy but also cross-component correspondence, for example, the alignment between bars and axis ticks.
%From this structure, it builds a chart dependency graph, in which nodes represent components, primitives, and editable attributes, and edges encode hierarchical containment and cross-component correspondences that should be preserved during editing.
%Our system then uses an LLM to interpret user intent over this graph and generate structured edit plans subject to these dependency constraints. 
%This design supports both precise local edits within a semantic component like recoloring a series, and more complex global edits that require coordinated modifications across multiple components, such as synchronizing series colors with legend markers or adjusting inter-bar spacing together with axis ticks and labels.


% ================================================
% \textbf{Paragraph 5: Evaluations}

% Quantitative and qualitative results of reconstruction accuracy, Ablation study, Qualitative results of editing, User study
% ================================================

After building the whole framework, 
We evaluate the proposed system from both reconstruction and downstream utility perspectives. Quantitatively, we measure reconstruction fidelity and conduct ablation studies to assess the impact of SVG normalization and post-training. Qualitatively, we examine the quality of semantic decomposition and the expressiveness of supported editing operations. The results show that our method improves not only visual faithfulness of reconstructed charts, but also their usefulness for downstream editing.


% ================================================
% \textbf{Paragraph 6: Contributions}
% ================================================

In summary, our contributions are threefold.
\begin{itemize}
    \item We investigate the practical challenge of automated chart editing, highlighting its critical importance for the timely adaptation of charts to evolving requirements in real-world scenarios.
    \item We introduce a semantic chart editing pipeline that recovers chart-level components from reconstructed SVGs and organizes them with a chart dependency graph to support reliable language-guided editing, including both group-wise local modifications and coordinated global updates across multiple related components.
    \item We investigate the practical challenge of automated chart editing, highlighting its critical importance for the timely adaptation of charts to evolving requirements in real-world scenarios.
    \item We present a systematic evaluation of chart recovery and editing, demonstrating that recovered charts are not only visually faithful but also practically useful for downstream editing tasks.
\end{itemize}


==> tables/CSG_component.tex <==
\begin{table}[t]
\centering
\caption{\new{Component extraction on VisAnatomy~\cite{chen2025visanatomy}, comparing
our method against DIVI~\cite{snyder2023divi} on type-level F1 and count accuracy
(Cnt.\ Acc.). Higher is better for all metrics.}}
\label{tab:csg_component}
\setlength{\tabcolsep}{5pt}
\new{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Component} &
\multicolumn{2}{c}{Type F1 $\uparrow$} &
\multicolumn{2}{c}{Cnt.\ Acc.\ $\uparrow$} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
 & Ours & DIVI & Ours & DIVI \\
\midrule
Mark       & \textbf{0.999} & 0.902 & \textbf{0.649} & 0.455 \\
Axis-tick  & \textbf{0.865} & 0.573 & \textbf{0.450} & 0.296 \\
Axis-label & \textbf{0.014} & 0.012 & \textbf{0.002} & 0.002 \\
Legend     & \textbf{0.420} & 0.307 & \textbf{0.143} & 0.069 \\
Title      & \textbf{0.113} & 0.045 & \textbf{0.041} & 0.015 \\
\midrule
Average    & \textbf{0.482} & 0.368 & \textbf{0.257} & 0.167 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/ablate_grpo.tex <==
\begin{table}[t]
\centering
\caption{Ablation on rendering-aware GRPO using the 4B model. Higher is better for PSNR, SSIM, Foreground IoU ($\mathrm{IoU}_{\mathrm{fg}}$), and Edge Consistency, while lower is better for LPIPS and Failure Rate.}
\label{tab:ablation_grpo}
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.12}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cccccc}
\toprule
\textbf{Variant}
& \textbf{PSNR} $\uparrow$
& \textbf{SSIM} $\uparrow$
& \textbf{LPIPS} $\downarrow$
& $\mathbf{IoU}_{\mathbf{fg}} \uparrow$
& \textbf{Edge Cons.} $\uparrow$
& \textbf{Failure Rate} $\downarrow$ \\
\midrule
SFT            & 6.8122 & 0.4672 & 0.6263 & 0.3771 & 0.2717 & 0.027 \\
GRPO w/o IoU   & 7.0908 & 0.4824 & 0.6185 & 0.3668 & 0.2794 & 0.009 \\
GRPO full      & \textbf{7.3115} & \textbf{0.4942} & \textbf{0.6033} & \textbf{0.3810} & \textbf{0.2858} & \textbf{0.000} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/ablate_token.tex <==
\begin{table}[t]
\centering
\caption{Ablation on chart SVG grammar tokens using the 4B model. Results are reported on the VisAnatomy test set. Higher is better for PSNR, SSIM, Foreground IoU ($\mathrm{IoU}_{\mathrm{fg}}$), and Edge Cons., while lower is better for LPIPS and Failure Rate.}
\label{tab:ablation_tokens}
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.12}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cccccc}
\toprule
\textbf{Variant}
& \textbf{PSNR} $\uparrow$
& \textbf{SSIM} $\uparrow$
& \textbf{LPIPS} $\downarrow$
& $\mathbf{IoU}_{\mathbf{fg}} \uparrow$
& \textbf{Edge Cons.} $\uparrow$
& \textbf{Failure Rate} $\downarrow$ \\
\midrule
w/o SVG tokens & 12.2325 & 0.6028 & 0.6358 & 0.1801 & \textbf{0.2585} & 0.148 \\
w/ SVG tokens  & \textbf{12.4000} & \textbf{0.6249} & \textbf{0.6303} & \textbf{0.1843} & 0.2579 & \textbf{0.109} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/recon_acc_dataset.tex <==
% ============================================================
% Table 1: Numerical Accuracy by Dataset
% ============================================================
\begin{table}[t]
\centering
\caption{Numerical accuracy by dataset. For each dataset, we report decoding rate (Dec.) and numerical accuracy among decodable samples (Acc., n = number of decodable samples). N/A indicates n $<$ 10; --- indicates no SVG output or no available samples.}
\label{tab:numerical_by_dataset}
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Model}}
& \multicolumn{2}{c|}{\textbf{ChartBlocks}}
& \multicolumn{2}{c|}{\textbf{Fusion}}
& \multicolumn{2}{c|}{\textbf{Plotly}}
& \multicolumn{2}{c}{\textbf{VisAnatomy}} \\
& \textbf{Dec.} & \textbf{Acc.}
& \textbf{Dec.} & \textbf{Acc.}
& \textbf{Dec.} & \textbf{Acc.}
& \textbf{Dec.} & \textbf{Acc.} \\
\midrule
\rowcolor{gray!20}
Adobe Illustrator\textsuperscript{$\dagger$}
& \new{0} & \new{N/A} & \new{0} & \new{N/A} & \new{0} & \new{N/A} & \new{0} & \new{N/A} \\
\midrule
StarVector~\cite{rodriguez2025starvector}
& \new{0} & \new{N/A} & \new{0} & \new{N/A} & \new{0} & \new{N/A} & \new{---} & \new{---} \\
OmniSVG~\cite{yangomnisvg}
& \new{0.0762} & \new{N/A} & \new{0.0085} & \new{N/A} & \new{0.0400} & \new{N/A} & \new{---} & \new{---} \\
GPT-4o
& \new{0.7345} & \new{0.1466} & \new{\textbf{0.4651}} & \new{0.2067} & \new{0.4941} & \new{0.1853} & \new{---} & \new{---} \\
GPT-o3
& \new{0.6339} & \new{0.2503} & \new{0.3281} & \new{\textbf{0.3327}} & \new{0.5349} & \new{0.2294} & \new{0.4737} & \new{\textbf{0.3042}} \\
Gemini 2.5
& \new{0.8053} & \new{0.2245} & \new{0.3178} & \new{0.2834} & \new{0.6395} & \new{\textbf{0.2740}} & \new{\textbf{0.5614}} & \new{0.2717} \\
\midrule
\ourmodel-8B
& \new{\textbf{0.8850}} & \new{\textbf{0.3018}} & \new{0.4109} & \new{0.1064} & \new{\textbf{0.6860}} & \new{0.2633} & \new{0.5246} & \new{0.2653} \\
\bottomrule
\end{tabular}
}
\end{table}

